Learning SO(3)-Invariant Semantic Correspondence via Local Shape Transform

Establishing accurate 3D correspondences between shapes stands as a pivotal challenge with profound implications for computer vision and robotics. However, existing self-supervised methods for this problem assume perfect input shape alignment, restricting their real-world applicability. In this work, we introduce a novel self-supervised Rotation-Invariant 3D correspondence learner with Local Shape Transform, dubbed RIST, that learns to establish dense correspondences between shapes even under challenging intra-class variations and arbitrary orientations. Specifically, RIST learns to dynamically formulate an SO(3)-invariant local shape transform for each point, which maps the SO(3)-equivariant global shape descriptor of the input shape to a local shape descriptor. These local shape descriptors are provided as inputs to our decoder to facilitate point cloud self- and cross-reconstruction. Our proposed self-supervised training pipeline encourages semantically corresponding points from different shapes to be mapped to similar local shape descriptors, enabling RIST to establish dense point-wise correspondences. RIST demonstrates state-of-the-art performances on 3D part label transfer and semantic keypoint transfer given arbitrarily rotated point cloud pairs, outperforming existing methods by significant margins.

==> assets/figures/tex/ablation_loss.tex <==
\begin{figure}[t]
    \begin{center}
        \includegraphics[width=0.5\linewidth]{assets/figures/png/ablation_loss_v2.png}
    \end{center}
      \caption{Ablation study on self-reconstruction (SR) and cross-reconstruction (CR) losses.
}
\label{fig:ablation_loss}
\end{figure}

==> assets/figures/tex/supp_acceptance.tex <==
\begin{figure}[h]
    \begin{center}
        \includegraphics[width=\linewidth]{assets/figures/png/acceptance_email.png}
    \end{center}
\label{fig:supp_acceptance}
\end{figure}

==> assets/figures/tex/supp_pck_keypointnet_i.tex <==
\begin{figure}[h]
    \begin{center}
        \includegraphics[width=1.0\linewidth]{assets/figures/png/kpn_i_so3_v3.png}
    \end{center}
      \caption{\textbf{Correspondence accuracy for 12 categories in the KeypointNet dataset.}
}
\label{fig:supp_pck}
\end{figure}

==> assets/figures/tex/supp_qual_part_label_transfer_guitar.tex <==
\begin{figure*}[h]
    \begin{center}
        \includegraphics[width=\linewidth]{assets/figures/pdf/supp_qual_part_guitar.pdf}
    \end{center}
      \caption{\textbf{Qualitative results of part label transfer on the guitar class in the ShapeNet part dataset~\cite{shapenetpart}.} Note that the input shapes were arbitrarily rotated, differently for each target column, but have been aligned for better visibility of part label transfer results.
      \methodName shows to outperform CPAE~\cite{cheng2021learning} consistently, showing a high resemblance to ground truth results.
}
\label{fig:supp_part_guitar}
\end{figure*}

==> assets/tables/ablation_ftm_equi.tex <==
\begin{table}
\centering

\begin{tabular}{c c c c c c}
\toprule
Equi. Enc. & Feature & Intermediate rep. & Equi. Dec.  & I  & SO(3) \\
\midrule
X  &  Global & Non-equi. UV & X & CPAE & CPAE \\
\midrule
O  & Global   &  Inv. UV & X &cho13 & cho13 \\
O  & Pointwise  & Inv. UV & X & cho14 & cho14 \\
O  & Pointwise  & Inv. FTM & X & cho6 & cho16 \\
O & Pointwise  & Inv. FTM & X & Ours & Ours \\
\bottomrule

\end{tabular}
\caption{
\textbf{Ablation study on SO(3)-equivariance and intermediate representation.} 
\textit{Equi. Enc.} and \textit{Equi. Dec.} shows whether SO(3)-equivariant layers were used for the Encoder and Decoder, respectively.
The \textit{Feature} column shows the type of feature the Encoder uses to yield intermediate representations.
UV refers to coordinates $\in \mathbb{R}^{N \times 3}$ in the UV space, while FTM refers to our proposed Feature Transformation Matrices.
The first row corresponds to CanonicalPAE~\cite{}, and we show that each step towards \methodName's final design choice show performance improvements.
}

\label{tbl:ablation_ftm_equi}

\end{table}



==> assets/tables/ablation_reconstruction.tex <==
\begin{table}
    \centering
    \begin{tabular}{cccc}
    \toprule
    Self-reconstruction & Cross-reconstruction & I & SO(3) \\
    \midrule
    o & o & Ours & Ours \\
    
    o & x & cho16 & cho6 \\
    
    x & o & cho6 & cho6 \\
    \bottomrule
    \end{tabular}

\caption{
\textbf{Ablation study on shape reconstruction of \methodName.} \seungwook{Short discussion of results.}
}
\label{tbl:ablation_reconstruction}
\end{table}

==> assets/tables/rebuttal_aligned_shapenetpart.tex <==
\centering
\scalebox{0.46}{
% Create your table here
\begin{tabular}{lrccc}
\toprule
IoU & \#Para. & Lat.(ms) & Airplane & Chair \\
\midrule
CPAE & 2.1 M & 10.5 & 17.0 & 24.5 \\
~+ PCA & 2.1 M & 10.9 & 23.3 & 24.8 \\
~+ VN-SPD & 19.5 M & 15.8 & \textbf{53.6} & 51.8 \\
RIST & 5.9 M & 11.2 & 51.2 & \textbf{58.3} \\
\bottomrule
\end{tabular}
}
\label{tab:rebuttal_aligned_shapenetpart}

==> assets/tables/rebuttal_sc3k.tex <==
% \begin{wraptable}{r}{0.43\linewidth} 
% \vspace{-0.4cm}
%     \centering
%     \vspace{1.5mm}
%     \scalebox{0.6}{
%     \hspace{-1cm}
%        \begin{tabular}{lccc}
%                 \toprule

%                 DAS & Airplane & Car & Chair \\
                
%                 \midrule

%                 SC3K-10kp & 81.3 & 73.8 & \textbf{86.2} \\
%                 RIST (ours) & \textbf{82.4} & \textbf{76.9} & 81.8 \\
%                 \midrule
%                 \midrule
%                 IoU & Airplane & Car & Chair \\
                
%                 \midrule

%                 SC3K-2048kp & 22.3 & 23.0 & 24.7 \\
%                 RIST (ours) & \textbf{51.2} & \textbf{48.0} & \textbf{58.3} \\
%                 \bottomrule
%         \end{tabular}    
%          }
%         \vspace{-3mm}
%         \label{tbl:rebuttal_das_sc3k}
% \end{wraptable}


\begin{figure}[h]
    \vspace{-4mm}
    \begin{minipage}{0.46\linewidth}
        \centering
        \footnotesize
        \begin{adjustbox}{width=\linewidth,center}
        \begin{tabular}{lccc}
            \toprule
            DAS & Airplane & Car & Chair  \\ 
            \midrule
            SC3K-10kp & 81.3 & 73.8 & \textbf{86.2} \\
            RIST (ours) & \textbf{82.4} & \textbf{76.9} & 81.8 \\
            \bottomrule
        \end{tabular}
        \end{adjustbox}
        \label{tbl:rebuttal_das_sc3k}
    \end{minipage}%
    \hspace{0.4em}
    \begin{minipage}{0.48\linewidth}
        \centering
        \footnotesize
        \begin{adjustbox}{width=\linewidth,center}
        \begin{tabular}{lccc}
            \toprule
            IoU & Airplane & Car & Chair  \\ 
            \midrule
            SC3K-2048kp & 22.3 & 23.0 & 24.7 \\
            RIST (ours) & \textbf{51.2} & \textbf{48.0} & \textbf{55.0} \\
            \bottomrule
        \end{tabular}
        \end{adjustbox}
        \label{tbl:rebuttal_iou_sc3k}
    \end{minipage}
    \vspace{-4mm}
\end{figure}

==> assets/tables/rebuttal_scanobjectnn.tex <==
\begin{wraptable}{r}{0.18\textwidth} 
\vspace{-4mm}
    \centering
    \scalebox{0.7}{
    \hspace{-10mm}
       \begin{tabular}{lccc}
                \toprule

                IoU & Bag & Chair & Table \\
                \midrule
                \midrule
                \multicolumn{4}{l}{\textit{Trained on ShapeNetPart}} \\ 
                \midrule
                CPAE & 85.7 & 23.9 & 42.2 \\
                RIST & \textbf{85.8} & \textbf{37.9} & \textbf{45.4} \\
                \midrule
                \multicolumn{4}{l}{\textit{Trained on Bag of ScanObjectNN}} \\ 
                \midrule
                CPAE$_\text{Bag}$ & 86.2 & 23.7 & 41.6 \\
                % CPAE$_\text{Chair}$ & - & - & - \\
                % CPAE$_\text{Table}$ & - & - & - \\
                RIST$_\text{Bag}$ & \textbf{87.6} & \textbf{29.8} & \textbf{48.2} \\
                % RIST$_\text{Chair}$ & - & - & - \\
                % RIST$_\text{Table}$ & - & - & - \\
                \bottomrule
        \end{tabular}
         }
        \label{tbl:rebuttal_scanobjectnn}
    \vspace{-4mm}
\end{wraptable}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> sections/02_problemsetup.tex <==
\section{Problem setup}
\label{sec:problem_setup}

\seungwook{Revise the text below to consider rotated and partial point clouds.}
Given two point clouds, $P$ and $Q$, both subsets of $\mathbb{R}^3$, the objective is to determine a dense correspondence between them, denoted by a set of point pairs $(p, q)$, such that $p \in P$ and $q \in Q$. 
This problem can be formulated mathematically as follows:

\begin{equation}
\begin{split}
& \text{Find } C : P \times Q \rightarrow \mathbb{R} \\
& \text{Subject to: } \\
& 1. \; \forall (p, q) \in C, \; p \in P \; \text{and} \; q \in Q \\
& 2. \; C \text{ minimizes an objective function } \mathcal{F}(C)
\end{split}
\end{equation}


In this formulation, the function $C$ represents the correspondence between points in the point clouds $P$ and $Q$, and $\mathcal{F}(C)$ is an objective function that quantifies the quality of the correspondence. The constraint (1) ensures that each point pair in $C$ consists of points from $P$ and $Q$. However, not all points in $P$ or $Q$ are required to have a corresponding point in the other point cloud, as the two point clouds may have different structures despite belonging to the same semantic category.

The primary challenge in solving this problem in realistic situations lies in the presence of partial information and random orientation of the point clouds. 
Specifically, given that $P$ and $Q$ may be incomplete or unaligned, it is necessary to develop a method that is robust to these variations and capable of determining accurate correspondences between the two point clouds.

Our proposed approach, \methodName, addresses this challenge by introducing a novel methodology that \seungwook{takes into account the intrinsic properties of the point clouds and efficiently establishes reliable and accurate correspondences between them, even in the presence of partial information and random orientation.}

==> supp_sections/iclr2024/a_pck.tex <==
\section{Additional results on KeypointNet with I/I and I/SO(3)}
\input{assets/figures/tex/supp_pck_keypointnet_i}

In this section, we provide the results of baseline methods~\citep{deprelle2019learning, yang2018foldingnet, liu2020learning, cheng2021learning} and ours evaluated on the KeypointNet dataset, but under the I/I setting used by previous methods, as shown in Figure~\ref{fig:supp_pck}.
Note that under the I/I setting, the input shape pairs are perfectly aligned both at train and test time - which is an unrealistic setting in practice.
For CPAE~\cite{cheng2021learning} and ours, we also include the results under the I/SO(3) setting to visualize the performance difference between the two evaluation settings.
It can be seen that while the drop in performance for CPAE from I/I to I/SO(3) setting is drastic, the difference is negligible in \methodName, demonstrating the robustness of our SO(3) correspondence establishment scheme against arbitrary rotations.
While \methodName is not always competitive on all datasets, it is impractical to expect perfectly aligned shapes in real-world situations; on the realistic setting of SO(3) evaluation, \methodName consistently shows the best results.

==> supp_sections/iclr2024/d_additional_qual.tex <==
\section{Additional qualitative results.}
We provide additional qualitative results which were not included in our manuscript due to space constraints, as shown in Figures~\ref{fig:supp_part_motor},~\ref{fig:supp_part_guitar}, and~\ref{fig:supp_part_airplane}.
It can be seen that under especially large intra-class variation, part segmentation label transfer using \methodName often yields unsatisfactory results.
\input{assets/figures/tex/supp_qual_part_label_transfer_motorcycle}
\input{assets/figures/tex/supp_qual_part_label_transfer_guitar}
\input{assets/figures/tex/supp_qual_part_label_transfer_airplane}
